Enumerative Lattice Algorithms in Any Norm via M-Ellipsoid Coverings

We give a novel algorithm for enumerating lattice points in any convex body, and give applications to several classic lattice problems, including the Shortest and Closest Vector Problems (SVP and CVP, respectively) and Integer Programming (IP). Our enumeration technique relies on a classical concept from asymptotic convex geometry known as the M-ellipsoid, and uses as a crucial subroutine the recent algorithm of Micciancio and Voulgaris (STOC 2010) for lattice problems in the l_2 norm. As a main technical contribution, which may be of independent interest, we build on the techniques of Klartag (Geometric and Functional Analysis, 2006) to give an expected 2^O(n)-time algorithm for computing an M-ellipsoid for any n-dimensional convex body. As applications, we give deterministic 2^{O(n)}-time and -space algorithms for solving exact SVP, and exact CVP when the target point is sufficiently close to the lattice, on n-dimensional lattices in any (semi-)norm given an M-ellipsoid of the unit ball. In many norms of interest, including all l_p norms, an M-ellipsoid is computable in deterministic poly(n) time, in which case these algorithms are fully deterministic. Here our approach may be seen as a derandomization of the "AKS sieve" for exact SVP and CVP (Ajtai, Kumar, and Sivakumar; STOC 2001 and CCC 2002). As a further application of our SVP algorithm, we derive an expected O(f*(n))^n-time algorithm for Integer Programming, where f*(n) denotes the optimal bound in the so-called "flatness theorem," which satisfies f*(n) = O(n^{4/3} \polylog(n)) and is conjectured to be f*(n)=\Theta(n). Our runtime improves upon the previous best of O(n^{2})^{n} by Hildebrand and Koppe (2010).

==> bound-enum.tex <==

\section{Bounding the CVP Enumeration Complexity}
\label{sec:enum-bounds}

The purpose of this section will be to establish interesting special cases where the algorithm Closest-Vectors performs
well in the worst case, by bounding the enumeration complexity.

\subsection{A Volume Bound}
\label{sec:volume-bound}

We will first show that the number of lattices points in $K$ acts like volume once $\mu(K,L) \leq 1$. This will allow us
to gain control over the main complexity term $G(K,L)$ of Closest-Vectors algorithm from the previous section.

\begin{lemma}
  \label{lem:lt-pts-vol}
  Let $K \subseteq \R^n$ be a convex body and let $L$ be an
  $n$-dimensional lattice. Then
  \begin{equation}
    \frac{\vol(K)}{\det(L)} \leq G(K,L) \leq \max \set{1, \mu(K,L)^n} 2^n \frac{\vol(K)}{\det(L)}
  \end{equation}
\end{lemma}

\begin{proof}
  Let $F$ denote any fundamental region of $L$. Then note that
  \begin{equation}
    \vol(K) = \int_F |L+x \cap K| dx
  \end{equation}
  Since $\vol(F) = \det(L)$, there must exist $x \in F$ such that $|L
  + x\cap K| \geq \frac{\vol(K)}{\det(L)}$ as needed.

  By shifting $K$, we may assume that $0 \in K$. Now let $\leq_{lex}$
  denote the standard lexicographic ordering on $\R^n$. Define
  \begin{equation}
    \mathcal{V}(L,K) = \set{x \in \R^n: 0 \in \CVP(-K,L,x), ~ 0 \leq_{lex} y ~ \forall ~ y \in \CVP(-K,L,x)}
  \end{equation}
  We claim that $\mathcal{V}(L,K)$ is a fundamental region of $L$,
  i.e. $\mathcal{V}(L,K)$ induces an $L$-periodic tiling of
  $\R^n$. Take $x,y \in L$, $x \neq y$. We must show that $x +
  \mathcal{V}(L,K) \cap y + \mathcal{V}(L,K) = \emptyset$.  Assume not
  and pick $z \in x + \mathcal{V}(L,K) \cap y +
  \mathcal{V}(L,K)$. Then we see that $x,y \in \CVP(-K,L,z)$, but then
  $x \leq_{lex} y$ and $y \leq_{lex} x$, a contradiction. Now take $z
  \in \R^n$. Let $x$ denote the lex least element of
  $\CVP(-K,L,z)$. Then clearly $z \in x + \mathcal{V}(L,K)$ as needed.

  By the definition of $\mathcal{V}(L,K)$ we see that $\mu(K,L) =
  \sup_{x \in \mathcal{V}(L,K)} \|x\|_{-K}$. Therefore for $x \in
  \mathcal{V}(L,K)$, we have that $0 \in x - \mu(K,L) K \Rightarrow x
  \in \mu(K,L) K$, hence $\mathcal{V}(L,K) \subseteq \mu(K,L) K$.

  Now we note that it suffices to prove the theorem when $\mu(K,L)
  \leq 1$, i.e. when $\mathcal{V}(K,L) \subseteq K$. Now take $x \in
  \R^n$. We wish to bound $|K \cap L + x|$. Since $\mathcal{V}(K,L)
  \subseteq K$, we note that for $y \in K \cap L + x$, we have that
  \begin{equation}
    y + \mathcal{V}(K,L) \subseteq K + \mathcal{V}(K,L) \subseteq K + K = 2K
  \end{equation}
  Furthermore, since $\mathcal{V}(K,L)$ is a fundamental region of
  $L$, we have that $\vol(\mathcal{V}(K,L)) = \det(L)$, and so
  \begin{equation}
    \vol(2K) \geq \vol\left(\bigcup_{y \in L+x \cap K} y + \mathcal{V}(K,L)\right) = |L+x \cap K| ~
    \vol(\mathcal{V}(K,L)) = |L+x \cap K| ~ \det(L)
  \end{equation}
  Hence $|L+x \cap K| \leq \frac{\vol(2K)}{\det(L)} = 2^n
  \frac{\vol(K)}{\det(L)}$.
\end{proof}

Now we remember that when running the Closest-Vectors algorithm on a body $K$, lattice $L$, and target $t$ the main
complexity term is $G(d_K(L,x) ~K, L)$. By definition we know that for all $x \in \R^n$, $d_K(L,x) \leq \mu(K,L)$.
Applying Lemma $\ref{lem:lt-pts-vol}$ above, we get that on any $x \in \R^n$, Closest-Vectors(K,L,x) runs time at most
\begin{equation}
2^{O(n)} G(\mu(K,L) K, L) \leq 2^{O(n)} \frac{\vol(\mu(K,L) K)}{\det(L)} 
                          \leq 2^{O(n)} \mu(K,L)^n \frac{\vol(K)}{\det(L)}
\label{eq:cvp-worst-case}
\end{equation}

With the above, we reduce the question of bounding the worst case running time of Closest-Vectors to bounding the volume
of $K$ once it has been scaled to have covering radius $1$ with respect to $L$. We address quantity in the following
sections.

\subsection{A Simple Transference Theorem}
\label{sec:transference}

Here we prove a specialization of a transference theorem of Banaszczyk based on gaussian measures.
The classic flatness theorem states that for a convex body $K$, and lattice $L$ the quantity
\begin{equation}
  \mu(K,L) \lambda_1((K-K)^*, L^*) \leq f(n)
\end{equation}
where $f(n)$ is a function depending only on dimension. The best known bounds for $f(n)$ come from the work of
Banaszczyk et al $\cite{Bana96,Bana99}$, and are based on estimate 
\begin{equation}
\mu(K,L) \lambda_1((K-K)^*, L^*) 
         \leq \inf_{\substack{T: \R^n \rightarrow \R^n \\ \text{$T$ affine invertible}}} l_2(TK)l_2((TK)^*)
\label{eq:transf-ll}
\end{equation}
The right hand side is the classical $l$-$l^*$ estimate in the Local Theory of Banach Spaces. For symmetric bodies it
can be shown that right hand side is bounded $O(n \log n)$ (see \cite{Pis89}) and for general bodies can be bounded by
$O(n^{\nicefrac{4}{3}}\log^{c} n)$ (see \cite{R00}).

In this section, we give a simple proof of ``half'' of the above inequality which will allow us to specialize our
analysis to the class of $\tau$-intrinsically smooth lattices.

\begin{theorem}
  \label{thm:easy-transference}
  Let $K \subseteq \R^n$ be a convex body and let $L \subseteq \R^n$
  be an $n$ dimensional lattice. Then for all $\eps \in (0,1)$, we
  have
  \begin{equation}
    \mu(K,L) \leq \frac{1+\eps}{1-\eps} ~ 2 ~ \eta_{\eps}(L) \inf_{x \in K} l_1(K-x)
  \end{equation}
\end{theorem}

Before proving the theorem we need a few definitions and simple facts.
For a countable subset $A \subseteq \R^n$, we define
\begin{equation}
  \sigma_{s,c}(A) = \sum_{x \in A} e^{-\frac{1}{2}\|\frac{x-c}{s}\|^2}
\end{equation}

We define the discrete gaussian distribution $D_{L,s,c}$ supported on
$L$ such that for $A \subseteq L$
\begin{equation}
  D_{L,s,c}(A) = \frac{\sigma_{s,c}(A)}{\sigma_{s,c}(L)}
\end{equation}

\begin{lemma}[{\cite[Lemma
    4.1]{DBLP:journals/siamcomp/MicciancioR07}}]
  Let $L \subseteq \R^n$ be an $n$-dimensional lattice and take $s
  \geq \eta_{\eps}(L)$. Then for all $c \in \R^n$, we have that
  \begin{equation}
    (1-\eps) \frac{(2\pi)^{\nicefrac{n}{2}}s^n}{\det(L)} \leq \sigma_{s,c}(L) 
    \leq (1+\eps) \frac{(2\pi)^{\nicefrac{n}{2}}s^n}{\det(L)}
  \end{equation}
  Furthermore $~ \sup_{c \in \R^n} ~ \sigma_{s,c}(L) =
  \sigma_{s,0}(L)$.
  \label{lem:smooth-lat}
\end{lemma}

From Lemma~\ref{lem:smooth-lat} we will be able to conclude that the
discrete Gaussian looks ``almost'' like the continuous Gaussian above
the smoothing parameter.  We make this precise in the following simple
lemma, which says that if we convolve a discrete Gaussian with a
continuous Gaussian, we get back a distribution very close to a
continuous gaussian in density.

\begin{lemma}
  Let $L \subseteq \R^n$ be an $n$-dimensional lattice and take $s
  \geq \eta_{\eps}(L)$. Let $X$ be distributed as $D_{L,s,c}$ and $Y$
  be distributed as $N(0,s^2\Id_n)$. Then for all $x \in \R^n$, we
  have that
  \begin{equation}
    \frac{1-\eps}{1+\eps} ~ (2\sqrt{\pi}s)^{-n} e^{-\nicefrac{1}{2}\left\|\frac{x-c}{\sqrt{2}s}\right\|^2} ~ \leq ~
    \lim_{\eps \rightarrow 0} \frac{\Pr(X+Y \in x + \eps B_2^n)}{\vol(\eps B_2^n)} ~ \leq ~
    \frac{1+\eps}{1-\eps} ~ (2\sqrt{\pi}s)^{-n} e^{-\nicefrac{1}{2}\left\|\frac{x-c}{\sqrt{2}s}\right\|^2}
  \end{equation}
  \label{lem:gauss-smooth}
\end{lemma}

\begin{proof}
  Let $c' = \frac{c+x}{\sqrt{2}}$. Now we have that
  \begin{align}
    \begin{split}
      \lim_{\eps \rightarrow 0} \frac{\Pr(X+Y \in x + \eps
        B_2^n)}{\vol(\eps B_2^n)} &= \frac{1}{\sigma_{s,c}(L) (\sqrt{2\pi}~ s)^n}
      \sum_{y \in L} e^{-\nicefrac{1}{2}\|\frac{y-c}{s}\|^2} e^{-\nicefrac{1}{2}\|\frac{x-y}{s}\|^2} \\
      &= \frac{1}{\sigma_{s,c}(L) (\sqrt{2\pi}~ s)^n} ~
      e^{-\nicefrac{1}{2} \left\|\frac{x-c}{\sqrt{2} s}\right\|^2}
      \sum_{y \in L} e^{-\nicefrac{1}{2}\left\|\frac{y-\nicefrac{(c+x)}{2}}{\nicefrac{s}{\sqrt{2}}}\right\|^2} \\
      &= \frac{\sigma_{\nicefrac{s}{\sqrt{2}}, c'}(L)}{\sigma_{s,c}(L)
        (\sqrt{2\pi}~ s)^n} ~ e^{-\nicefrac{1}{2}
        \left\|\frac{x}{\sqrt{2} s}\right\|^2}
      \label{eq:gauss-smooth-1}
    \end{split}
  \end{align}
  Since $s, \nicefrac{s}{\sqrt{2}} \geq \eta_{\eps}(L)$, by Lemma
  \ref{lem:smooth-lat} we have that
  \begin{align}
    \begin{split}
      (1-\eps) \frac{(\sqrt{\pi}~s)^n}{\det(L)} \leq
      \sigma_{\nicefrac{s}{\sqrt{2}}, c'}(L)
      \leq (1+\eps) \frac{(\sqrt{\pi}~s)^n}{\det(L)} \\
      (1-\eps) \frac{(\sqrt{2\pi}s)^n}{\det(L)} \leq \sigma_{s,c}(L) \leq (1+\eps) \frac{(\sqrt{2\pi}s)^n}{\det(L)} \\
    \end{split}
  \end{align}

  Combining the above inequalities with $\ref{eq:gauss-smooth-1}$
  yields the result.
\end{proof}

\noindent We can now prove our transference theorem.

\begin{proof}[Proof of Theorem~\ref{thm:easy-transference}]
  To bound $\mu(K,L)$ we must find $t \geq 0$ such that $\forall c \in
  \R^n$, $c + tK \cap L \neq \emptyset$. Since the previous property
  is invariant under shifts of $K$, we may pick $x \in K$ and work
  with $K-x$. Hence we may assume that $0 \in K$.

  Now pick $c \in \R^n$. Let $s = \sqrt{2} \eta_{\eps}(L)$. Let $X$ be
  distributed as $D_{L,s,c}$, and let $Y$ be distributed
  $N(0,s^2\Id_n)$. Since $0 \in K$, the function $\|\cdot\|_K$ is
  convex, therefore by Jensen's inequality we get that
  \begin{align}
    \begin{split}
      \E[\|X-c+Y\|_K] &= \sum_{x \in L} \E[\|x-c+Y\|_K]\Pr(X = x) \geq \sum_{x \in L} \|x-c+\E[Y]\|_K\Pr(X = x) \\
      &= \sum_{x \in L} \|x-c\|_K \Pr(X = x) = \E[\|X-c\|_K]
    \end{split}
  \end{align}
  Since $s \geq \sqrt{2} \eta_{\eps}(L)$, we know that the density
  function of $X+Y$ is a function $g(z): \R^n \rightarrow \R_+$ such
  that
  \begin{equation}
    \frac{1-\eps}{1+\eps} ~ (2\sqrt{\pi}s)^{-n} e^{-\pi\left\|\frac{z-c}{\sqrt{2}s}\right\|^2} ~ \leq ~
    g(z) ~ \leq ~
    \frac{1+\eps}{1-\eps} ~ (2\sqrt{\pi}s)^{-n} e^{-\pi\left\|\frac{z-c}{\sqrt{2}s}\right\|^2}
  \end{equation}
  Therefore, we have that
  \begin{align}
    \begin{split}
      \E[\|X-c\|_K] &\leq \E[\|X+Y-c\|_K] = \int_{\R^n} \|z-c\|_K g(z) dx = \int_{\R^n} \|z\|_K g(z+c) dx \\
      &\leq \frac{1+\eps}{1-\eps} (2\sqrt{\pi}s)^{-n} ~ \int_{\R^n}
      \|z\|_K e^{-\nicefrac{1}{2}\left\|\frac{z}{\sqrt{2}s}\right\|^2}
      = \frac{1+\eps}{1-\eps} ~ (2\pi)^{-\nicefrac{n}{2}} \int_{\R^n} \|\sqrt{2}s z\|_K e^{-\nicefrac{1}{2} \left\| z \right\|^2} \\
      &= \frac{1+\eps}{1-\eps} ~ \sqrt{2} ~ s ~ l_1(K) = \frac{1+\eps}{1-\eps} ~ 2 ~ \eta_{\eps}(L) ~ l_1(K) \\
    \end{split}
  \end{align}
  Let $t = \frac{1+\eps}{1-\eps} ~ \sqrt{2} ~ s ~ l_1(K)$. Since
  $\E[\|X-c\|_K] \leq t$, there must exists $x \in L$ such that
  $\|x-c\|_K \leq t \Rightarrow c + tK \cap L \neq \emptyset$. Since
  the choice of $c$ was arbitrary, we have that $\mu(K,L) \leq
  t$. Next, since we have the freedom to re-center $K$, we can achieve
  $\inf_{x \in K} l_1(K-x)$. The theorem thus follows.
\end{proof}

The above gives us a simple formulation of half of Banaszczyk's transference theorem. To get the other half, what is
required is to bound $\eta_{\eps}(L)$ as a function $\lambda_1((K-K)^*,L^*)$. This is explicitly done for
different bodies $K$ in each of~\cite{banaszczyk93:_new,DBLP:journals/dcg/Banaszczyk95,Bana96}, where in full generality
it is approached via Talagrand's theorem on majorizing measures. The main difference here is that for us
$\eta_{\eps}(L)$ is in fact a ``norm-free'' concept depending only on the lattice, whereas in Banaszczyk's work this
concept generally appears entangled with a specific norm.

\subsection{Round Bodies and Smooth Lattices}
\label{sec:cvp-round-smooth}

Here we show how to bound the term in
Equation~\eqref{eq:cvp-worst-case}, i.e., the main complexity term of
the Closest-Vectors algorithm. The bounds are completely general, and
can be arbitrarily large, but they help establish an interesting class
of cases where the bounds are quite reasonable.

\begin{theorem}
  \label{thm:sr-transf}
  Let $K \subseteq \R^n$ be a $\rho$-round convex body with $b(K) =
  0$, and let $L \subseteq \R^n$ be an $\tau$-intrinsically smooth
  $n$-dimensional lattice.  Then
  \begin{equation}
    \frac{\vol(\mu(K,L) K)}{\det(L)} \leq \inf_{x \in K} 
    \left(4 ~ \rho \cdot \tau \cdot \frac{l_1(K-x) \lambda_n(K)^{\nicefrac{1}{2}}}{L_K}\right)^n.
  \end{equation}
\end{theorem}

\begin{proof}
  First choose $x \in K$, and recenter $K$ around $x$. Hence as usual,
  we may assume that $0 \in K$. Since $L$ is $\tau$-intrinsically smooth, we have
  that
  \begin{equation}
    \eta_{\nicefrac{1}{3}}(L) \leq \tau \det(L)^{\frac{1}{n}}
  \end{equation}
  Now from Theorem \ref{thm:easy-transference}, we have that
  \begin{equation}
    \mu(K,L) \leq \frac{1+\nicefrac{1}{3}}{1-\nicefrac{1}{3}} ~ 2 ~ \eta_{\nicefrac{1}{3}}(L) l_1(K) \leq (2) ~ (2) ~ \tau
    \det(L)^{\frac{1}{n}} l_1(K) = 4 \tau \det(L)^{\frac{1}{n}} l_1(K)
  \end{equation}
  Now we note that
  \begin{equation}
    \vol(K) = \frac{\det(\cov(K))^\frac{1}{2}}{L_K^n} \leq \left(\frac{\lambda_1(K)^{\nicefrac{1}{2}}}{L_K}\right)^n \leq
    \left(\frac{\rho \lambda_n(K)^{\nicefrac{1}{2}}}{L_K}\right)^n
  \end{equation}
  Therefore we get that
  \begin{equation}
    \frac{\vol(\mu(K,L) K)}{\det(L)} \leq \frac{\vol(4 \tau \det(L)^{\frac{1}{n}} l_1(K) K)}{\det(L)}
    \leq (4 \tau l_1(K))^n \vol(K) 
    \leq \left(4 ~ \rho \cdot \tau \cdot \frac{l_1(K) \lambda_n(K)^{\nicefrac{1}{2}}}{L_K}\right)^n
  \end{equation}
  Since we picked the center $x \in K$ arbitrarily, we may achieve
  $\inf_{x \in K} l_1(K-x)$.
\end{proof}

\begin{lemma}
  \label{lem:gauss-inc}
  Let $f:\R \rightarrow \R$ be a convex function. Let $X_1,X_2$ be
  independent random variables distributed as $N(0,s_1)$ and
  $N(0,s_2)$ respectively, where $s_1 \leq s_2$. Then we have that
  \begin{equation}
    \E[f(X_1)] \leq \E[f(X_2)]
  \end{equation}
\end{lemma}

\begin{proof}
  Pick $s_3 > 0$ such that $s_1^2 + s_3^2 = s_2^2$, and let $X_3$ be
  independent of $X_1,X_2$ and distributed as $N(0,s_3)$. Then by the
  properties of the gaussian distribution, we know that $X_1 + X_3
  \equiv_{d} X_2$, hence
  \begin{equation}
    \E[f(X_2)] = \E[f(X_1+X_3)]
  \end{equation}
  Now by Jensen's inequality, since $f$ is convex, we have that
  \begin{equation}
    \E[f(X_1+X_3)] \geq \E[f(X_1 + \E[X_3])] = \E[f(X_1)]
  \end{equation}
  completing the proof.
\end{proof}

\begin{lemma} Let $K \subseteq \R^n$ be a convex body with $b(K) =
  0$. Let $C = \cov(K)^{-\nicefrac{1}{2}}$. Then
  \begin{equation}
    \sup_{\substack{T:\R^n \rightarrow \R^n \\ \text{T linear invertible}}} \frac{l_1(TK) \lambda_n(TK)^{\nicefrac{1}{2}}}{L_{TK}} = 
    \frac{l_1(CK) \lambda_n(CK)^{\nicefrac{1}{2}}}{L_K}
  \end{equation}
  Hence, the above quantity is maximized when $K$ is in isotropic
  position.
  \label{lem:iso-worst-case}
\end{lemma}
\begin{proof}
  Since $b(K) = 0$, we have that $0 \in K$ and hence $\|\cdot\|_K$ is
  a semi-norm. First we note that $L_K = L_{TK}$ for any affine
  transformation $T$, hence the term in the denominator is constant
  and therefore immaterial to the maximization. Now for any scaling $s
  > 0$, we note that $l_1(sK) = \frac{1}{s}l_1(K)$ (since $\|x\|_{sK}
  = \frac{1}{s} \|x\|_K$), and $\lambda_n(sK)^{\nicefrac{1}{2}} = s
  \lambda_n(K)^{\nicefrac{1}{2}}$. Therefore the quantity we wish to
  maximize is scale invariant. After an appropriate scaling we may
  therefore assume that $\lambda_n(K) = 1$. Next for any orthogonal
  transformation $R:\R^n \rightarrow \R^n$, we have that
  \begin{equation}
    l_1(RK) = \int_{\R^n} \|x\|_{RK} d\gamma(x) = \int_{\R^n} \|Rx\|_{RK} d\gamma(Rx) = \int_{\R^n} \|x\|_K d\gamma(x) = l_1(K)
  \end{equation}
  and
  \begin{equation}
    \lambda_n(RK) = \inf_{v \in S^{n-1}} v^t \cov(RK) v = \inf_{v \in S^{n-1}} v^t R \cov(K) R^t v =
    \inf_{v \in S^{n-1}} v^t \cov(K) v = \lambda_n(K)
  \end{equation}
  Therefore both quantities in the maximation are rotationally
  invariant. Hence after an appropriate rotation, since the matrix
  $\cov(K)$ is positive definite, we may assume that $\cov(K) =
  \mathrm{diag}(\lambda_1(K),\lambda_2(K),\dots,\lambda_n(K))$, where
  we know that $\lambda_1(K) \geq \lambda_2(K) \geq \dots \geq
  \lambda_n(K) = 1$. From here, we show that making $K$ isotropic only
  increases $l_1(K)$ while keeping $\lambda_n(K)$ the same, and
  therefore $l_1(K)\lambda_n(K)^{\nicefrac{1}{2}}$ increases.

  Now let
  \begin{equation}
    C = \cov(K)^{-\nicefrac{1}{2}} = \mathrm{diag}\left(\frac{1}{\lambda_1^{\nicefrac{1}{2}}(K)},\dots,\frac{1}{\lambda_n^{\nicefrac{1}{2}}(K)}\right)
  \end{equation}
  First note that $\cov(CK) = C\cov(K)C^t = \cov(K)^{-\nicefrac{1}{2}}
  \cov(K) \cov(K)^{-\nicefrac{1}{2}} = \Id_n$. Hence $\lambda_n(CK) =
  \lambda_n(\Id_n) = 1 = \lambda_n(K)$.

  \paragraph{Claim:} Let $T = \diag(a_1,\dots,a_n)$ where $0 < a_i
  \leq 1$, $1 \leq i \leq n$. Then $l_1(TK) \geq l_1(K)$.

  To show this, it suffices to prove the inequality for the linear
  transformation $T(x_1,\dots,x_n) = (a x_1, x_2, \dots, x_n)$ where
  $0 < a < 1$. Once this is shown, the general inequality is obtained
  by expressing a general $T$ as a composition of single coordinate
  scaling matrices and appying the inequality recursively. Now we have
  that
  \begin{align}
    \begin{split}
      l_1(TK) &= (2\pi)^{-\nicefrac{n}{2}} \int_{\R^n} \|x\|_{TK}
      e^{-\nicefrac{1}{2}\|x\|^2}
      =  (2\pi)^{-\nicefrac{n}{2}}|\det(T)| \int_{\R^n} \|Tx\|_{TK} e^{-\pi\|Tx\|^2} \\
      &= (2\pi)^{-\nicefrac{n}{2}} a \int_{\R^n} \|x\|_K
      e^{-\nicefrac{1}{2} a^2 x_1^2}
      e^{-\nicefrac{1}{2}(\sum_{i=2}^n x_i^2)} dx \\
      &= (2\pi)^{-\frac{n-1}{2}} \int_{\R^{n-1}}
      \left(\frac{a}{\sqrt{2\pi}} \int_\R \|(x_1,\dots,x_n)\|_K
        e^{-\nicefrac{1}{2} a^2 x_1^2} dx_1\right)
      e^{-\nicefrac{1}{2}(\sum_{i=2}^n x_i^2)} dx_2\dots dx_n
      \label{eq:wci-1}
    \end{split}
  \end{align}
  Now by Lemma \ref{lem:gauss-inc}, since
  $\|(\cdot,x_2,\dots,x_n)\|_K$ is a convex function of on $\R$ and $a
  \leq 1$, we see that
  \begin{equation}
    \frac{a}{\sqrt{2\pi}} \int_{\R} \|(x_1,x_2,\dots,x_n)\|_K e^{-\nicefrac{1}{2} a^2 x^2} dx_1 \geq \frac{1}{\sqrt{2\pi}} \int_\R \|(x_1,x_2,\dots,x_n)\| e^{-\nicefrac{1}{2} x_1^2}
  \end{equation}
  Plugging this back into (\ref{eq:wci-1}), we have that
  \begin{align}
    \begin{split}
      l_1(TK) &\geq (2\pi)^{-\frac{n-1}{2}} \int_{\R^{n-1}} \left((2\pi)^{-\nicefrac{1}{2}} \int_\R \|(x_1,\dots,x_n)\|_K e^{-\nicefrac{1}{2} x_1^2} dx_1\right)  e^{-\nicefrac{1}{2} (\sum_{i=2}^n x_i^2)}dx_2\dots dx_n \\
      & = \int_{\R^n} \|x\|_K d\gamma(x) = l_1(K)
    \end{split}
  \end{align}
  as needed.

  Now by construction, the matrix $C$ satisfies the conditions of the
  above claim, and hence $l_1(CK) \geq l_1(K)$.  Therefore
  $l_1(K)\lambda_n(K)^{\nicefrac{1}{2}} \leq
  l_1(CK)\lambda_n(CK)^{\nicefrac{1}{2}}$ as needed. Now we have shown
  that from any starting position, the quantity $l_1(K)
  \lambda_n(K)^{\nicefrac{1}{2}}$ only increases when we put $K$ in
  isotropic position. Given that the isotropic position $K$ is
  uniquely determined up to rotation, this proves the theorem.
\end{proof}

We will need the following fact about Gaussian random variable. For a
reference, see~\cite[Lemma 4.14]{Pis89}.

\begin{lemma}
  \label{lem:gauss-ub}
  Let $X_1,\dots,X_m$ denote a sequence of mean zero real valued
  gaussian random variables on a probability space $(\Omega,P)$.
  \begin{equation}
    \E\left[\max_{1 \leq i \leq m} |X_i|\right] \leq c\sqrt{1+\log m} \cdot \max_{1 \leq i \leq m} \sqrt{\E[X_i^2]}
  \end{equation}
  where $c > 0$ is an absolute constant.
\end{lemma}

We are now able to prove the two main technical lemmas required to prove Theorem $\ref{thm:cvp-smooth-lp}$ and
$\ref{thm:cvp-smooth-polytope}$.

\begin{lemma} Let $P$ be a $\rho$-round $m$-facet polytope and let $L \subseteq \R^n$ be an $\tau$-intrinsically smooth
$n$ dimensional lattice. Then
  \begin{equation}
    \frac{\vol(\mu(K,L) K)}{\det(L)} \leq c^n \left(\rho ~ \tau ~ \sqrt{\log m}\right)^n
  \end{equation}
  where $c > 0$ is an absolute constant.
  \label{lem:polytopes}
\end{lemma}
\begin{proof}
  Given Theorem $\ref{thm:sr-transf}$ and Lemma
  $\ref{lem:iso-worst-case}$, it suffices to prove that
  \begin{equation}
    \frac{l_1(P) \lambda_n(P)^{\nicefrac{1}{2}}}{L_P} \leq c \sqrt{\log m}
  \end{equation}
  when $P$ is in isotropic position, i.e. when $\cov(P) = \Id_n$ and
  $b(P) = 0$. Since $P$ is isotropic we have that $\lambda_n(P) = 1$.

  We now bound $l_1(K)$. Since $0 \in P$ and $P$ has $m$ facets, $P$
  can be represented as
  \begin{equation}
    P = \set{x \in \R^n: Ax \leq 1}
  \end{equation}
  where $A$ is an $m \times n$ matrix. Let $a_i$ denote the $i^{th}$
  row of $A$. It is a simple calculation to verify that for $x \in
  \R^n$, $\|x\|_P = \max_{1 \leq i \leq m} \pr{a_i}{x}$. By Theorem
  \ref{thm:sandwich}, since $P$ is isotropic, we know that
  \begin{equation}
    \sqrt{\frac{n+2}{n}}B_2^n \subseteq P \subseteq \sqrt{(n+2)n}B_2^n
  \end{equation}
  Since $B_2^n \subseteq P$, it follows that $\|x\|_P \leq \|x\| ~
  \forall ~ x \in \R^n \Leftrightarrow \|a_i\| \leq 1 ~ \forall ~ i
  \in \set{1,\dots,m}$.

  Let $X$ be distributed as $N(0,\Id_n)$. Then we see that
  \begin{equation}
    l_1(K) = \int_{\R^n} \|x\|_P d\gamma(x) = \int_{\R^n} \max_{1 \leq i \leq m} \pr{a_i}{x} d\gamma(x) = 
    \E\left[\max_{1 \leq i \leq m} \pr{a_i}{X}\right]
  \end{equation}
  For each $i$, we see that $\pr{a_i}{X} = \sum_{j=1}^n a_{ij}X_j$ is
  distributed as $N(0,\|a_i\|^2)$. Therefore, from Lemma
  \ref{lem:gauss-ub} we have that
  \begin{align}
    \begin{split}
      \E\left[\max_{1 \leq i \leq m} \pr{a_i}{X}\right] &\leq
      \E\left[\max_{1 \leq i \leq m} |\pr{a_i}{X}|\right]
      \leq c(1+\log m)^{\nicefrac{1}{2}} \max_{1 \leq i \leq n} \E[\pr{a_i}{X}^2]^{\nicefrac{1}{2}} \\
      &= c(1+\log m)^{\nicefrac{1}{2}} \max_{1 \leq i \leq n} \|a_i\|
      \leq c(1+\log m)^{\nicefrac{1}{2}}
    \end{split}
  \end{align}

  Now we need a lower bound on $L_K$. Among all convex bodies, the
  unit ball has the smallest isotropic constant (see~\cite{Ball88}
  or~\cite{B86}).  A direct computation yields then that $L_K \geq
  (2\pi e)^{-\nicefrac{1}{2}}(1+o(1))$.  Combining the above bounds,
  we get that
  \begin{equation}
    \frac{l_1(P) \lambda_n(P)^{\nicefrac{1}{2}}}{L_K} \leq c(1+\log m)^{\nicefrac{1}{2}}\sqrt{2\pi e}(1+o(1)) \leq c'
    \sqrt{\log m}
  \end{equation}
  where $c' > 0$ is an absolute constant.
\end{proof}

\begin{lemma} Take $p \geq 1$, and let $L \subseteq \R^n$ be an
  $\tau$-intrinsically smooth $n$-dimensional lattice. Then
  \begin{equation}
    \frac{\vol(\mu(B_p^n,L) B_p^n)}{\det(L)} \leq c^n \left(\tau
      \sqrt{\min \set{\log n, p}} \right)^n
  \end{equation}
  where $c > 0$ is an absolute constant.
  \label{lem:lp_balls}
\end{lemma}
\begin{proof}
  As in the previous corollary, it suffices to show that
  \begin{equation}
    \frac{l_1(B_p^n) \lambda_n(B_p^n)^{\frac{1}{2}}}{L_{B_p^n}} \leq c
    \sqrt{\min \set{\log n, p}}
  \end{equation}
  for a universal constant $c > 0$.

  A standard computation gives $\lambda_n(B_p^n) = \lambda_1(B_p^n)
  \approx n^{-\nicefrac{1}{p}}$ up to universal constants. For $1 \leq
  p \leq 2$, we note that
  \begin{align}
    \begin{split}
      l_1(B_p^n) &= \int_{\R^n} \|x\|_p d\gamma(x) \leq
      \left(\int_{\R^n} \|x\|_p^p d\gamma(x)\right)^{\nicefrac{1}{p}}
      = \left(\int_{\R^n} \sum_{i=1}^n x_i^p d\gamma(x)\right)^{\nicefrac{1}{p}} \\
      &\leq \left(\int_{\R^n} \sum_{i=1}^n x_i^2
        d\gamma(x)\right)^{\nicefrac{1}{p}} = n^{\nicefrac{1}{p}}
    \end{split}
  \end{align}
  As in the previous corollary, it suffices to use the bound
  $L_{B_p^n} \geq (2\pi e)^{-\nicefrac{1}{2}}(1+o(1))$.  Combining the
  above inequalities yields the desired result for $1 \leq p \leq 2$.

  For $p \geq 2$, we use a result of Schechtman and Zinn~\cite{SZ90},
  where Lemma 2 Part 4 gives that
  \begin{equation}
    l_1(B_p^n) \approx \sqrt{\min \set{\log n, p}} \cdot n^{\nicefrac{1}{p}}
  \end{equation}
  where the approximation is up to universal constants. This yields
  the result.
\end{proof}

\subsection{Distributions over Lattices}
\label{sec:random-lattice}

We begin with a simple lower bound on $\tau$-intrinsic smoothness.

\begin{lemma} Let $L \subseteq \R^n$ be an $n$-dimensional
  $\tau$-intrinsically smooth lattice.  Then $\tau \geq
  (1-\nicefrac{1}{n}) ~ \frac{1}{\sqrt{2\pi}}$.
  \label{lem:smooth-bound}
\end{lemma}
\begin{proof}
  Assume that $\tau < (1-\nicefrac{1}{n}) ~
  \frac{1}{\sqrt{2\pi}}$. Let $s = \tau \det(L)^{\frac{1}{n}}$. Then
  by Lemma $\ref{lem:smooth-lat}$ we have that
  \begin{align}
    \begin{split}
      \sigma_{s,0}(L) \leq
      (1+\nicefrac{1}{3})\frac{(2\pi)^{\nicefrac{n}{2}} s^n}{\det(L)}
      = \frac{4}{3} \frac{(2\pi)^{\nicefrac{n}{2}} \tau^n
        \det(L)}{\det(L)} \leq \frac{4}{3}
      \left(1-\frac{1}{n}\right)^n \leq \frac{4}{3e} < 1
    \end{split}
  \end{align}
  On the other hand, we have that
  \begin{equation}
    \sigma_{s,0}(L) = \sum_{x \in L} e^{-\nicefrac{1}{2}\|\frac{x}{s}\|^2} \geq e^{-\nicefrac{1}{2}\|\frac{0}{s}\|^2} = 1
  \end{equation}
  a clear contradiction.
\end{proof}

For natural distributions, a `random' lattice is $O(1)$-intrinsically
smooth with very high probability.  By the Gaussian heuristic, a
random $n$-dimensional lattice $L$ having determinant $1$ has dual
minimum distance (in the $\ell_{2}$ norm) $\Omega(\sqrt{n})$, which
implies that its smoothing parameter $\eta_{\epsilon}(L) = O(1)$ for
$\epsilon = 2^{-n}$, by~\cite[Lemma
3.2]{DBLP:journals/siamcomp/MicciancioR07}.  The Gaussian heuristic
can be made rigorous for natural distributions, such as the
Goldstein-Mayer distribution~\cite{goldstein03:_equid_of_hecke_point}
and the Haar measure over the group of lattices of determinant $1$.
We defer the details to the full version.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "svp-anynorm"
%%% End: 

